Unsupervised Context Aware Sentence Representation Pretraining for Multi-lingual Dense Retrieval

Recent research demonstrates the effectiveness of using pretrained language models (PLM) to improve dense retrieval and multilingual dense retrieval. In this work, we present a simple but effective monolingual pretraining task called contrastive context prediction~(CCP) to learn sentence representation by modeling sentence level contextual relation. By pushing the embedding of sentences in a local context closer and pushing random negative samples away, different languages could form isomorphic structure, then sentence pairs in two different languages will be automatically aligned. Our experiments show that model collapse and information leakage are very easy to happen during contrastive training of language model, but language-specific memory bank and asymmetric batch normalization operation play an essential role in preventing collapsing and information leakage, respectively. Besides, a post-processing for sentence embedding is also very effective to achieve better retrieval performance. On the multilingual sentence retrieval task Tatoeba, our model achieves new SOTA results among methods without using bilingual data. Our model also shows larger gain on Tatoeba when transferring between non-English pairs. On two multi-lingual query-passage retrieval tasks, XOR Retrieve and Mr.TYDI, our model even achieves two SOTA results in both zero-shot and supervised setting among all pretraining models using bilingual data.

==> 2022_naacl_draft/backup.tex <==
\iffalse
\ignore{
\section{Methodology}
This section proposes a constrastive learning framework for cross-lingual pretraining.

\subsection{The Contrastive Learning Framework}
Based on SimCLR, we propose a new contrastive learning 
framework to learn the sentence without parallel corpus.

\begin{itemize}
\item A transformer based encoder $f(\cdot)$ that learns the representation of input monolingual corpus $H_1=f(s_1)$ and $H_2=f(s_2)$. This encoder can be replaced by any model. We choose transformer to learn the sentence representation and use the representation of a mannually-inserted token [cls] as the vector of the sentence.

\item A nonlinear neural network projection head $g(\cdot)$ that maps the encoded augmentation $H_1$ and $H_2$ to the vector $z_1=g(H_1)$ and $z_2=g(H_2)$ to and new space. Adding a nonlinear projection head can significantly improve representation quality of images in SimCLR. Practically, the projection head is also essential to our model. It can force the encoder to learn task-independent representations.

\item A language-specific memory bank $M={M_i}$ that collect sentence representation output by projection head. The "language-specific" means that our memory bank will categorize these vectors by language. The memory bank is maintained in FIFO~(First-In-First-Out) manner. During each iteration, the representation $z_i$ as well as the network parameters $\theta$ are optimized via stochastic gradient descend. Then $z_i$ is added to $M$, and the oldest representation in the memory bank is deleted. 


\item A contrastive learning loss function defined for a contrastive prediction task, i.e., trying to predict positive augmentation pair ($\widetilde{s}_1$, $\widetilde{s}_2$) in the set {$\widetilde{s}$}. For example, two sentence in the same context form the positive pair, while all other instances from the same minibatch and memory bank are regarded as negative samples for them.  The contrastive learning loss has been tremendously used in previous work. The loss for a positive pair is defined as 

\begin{equation}
\resizebox{.9\hsize}{!}{
l(s_i,s_j)=-\log \frac{\exp(\cos(z_i,z_j)/\tau)}{\sum_{k=1}^{2N+M_{lg(i)}} \mathbbm{1}_{[k \ne i]} \exp(\cos (z_i,z_k)/\tau) }  \nonumber
}
\end{equation}

where $\mathbbm{1}_{[k \ne i]}$ is the indicator function to judge whether $k \ne i$, $\tau$ is a temperature parameter, $N$ is the size of minibatch, $M$ is the size of memory bank.  $\cos(u,v)=u^Tv/( \left\|u\right\|_2 \left\|v\right\|_2)$ denotes the cosine similarity of two vectors $u$ and $v$. The overall contrastive learning loss is defined as the sum of all positive pairs' loss in a minibatch:

\begin{equation}
\mathcal{L}_{CL}=\sum_{i=1}^{2N} \sum_{j=1}^{2N} m(i,j)l(i,j)  \nonumber
\end{equation}
where m(i,j) is a function returns 1 when i and j is a positive pair, returns 0 otherwise.

\end{itemize}
\subsection{The Context-Predictive Contrastive Learning}
Inspired by the continuous skip-gram model and continuous bag-of-words model, we propose a new contrastive learning manner based on predicting context. We  construct positive pair in a context window, and force the model to predict positive pair from numberous negative samples. 
Given a context window in a document, which contains $w$ sentences. We define the middle sentence $s_c$ as pivot sentence. Then we can extract other sentences $s_i$ in the window, and construct positive pairs \{$<s_c, s_i>$\}. The context-predictive contrastive loss can be written as:

\begin{equation}
\mathcal{L}_{ST}=\sum_{w}^{W} \sum_{i}^{w.l} \mathbbm{1}_{[c \ne i]}l(c, i)  \nonumber
\end{equation}
where $c$ is the index of pivot sentence in the window $w$, $\mathbbm{1}_{[c \ne i]}$ is the indicator function to judge whether $c \ne i$.
}
\fi

==> 2022_naacl_draft/sup.tex <==
\section{Supplementary Materials}
\label{sec:supplementary}
\begin{table*}[!h]
  \small
	\centering
	\resizebox{1\linewidth}{!}{
	\begin{tabular}{lccccccccccccccccccccc}
		\hline
		Task & Model & AR & BG & DE & EL & EN & ES & FR & HI & IT  & PT & RU & SW & TH & TR & UR & VI & ZH & AVG \\
				\hline
		\hline
        \multirow{4}{*}{MLQA}                       & M-BERT        & 50.9 & - & 63.8 & - & 80.5 & 67.1 & - & 47.9 & - &  - & - & - & - & - & - & 59.5 & 55.4 & 60.7 \\
		                                            & XLM-R$_{base}$         & 56.4 & - & 62.1 & - & 80.1 & 67.9 & - & 60.5 & - &  - & - & - & - & - & - & 67.1 & 61.4 & 65.1 \\
    		                                            & Unicoder& 57.8 & - & 62.7 & - & 80.6 & 68.6 & - & 62.7 & - &  - & - & - & - & - & - & 67.5 & 62.1 & 66.0 \\
		                                            &
		                            CCPC& 58.2 & - & 62.6 & - & 80.4 & 68.8 & - & 63.0 & - &  - & - & - & - & - & - & 68.1 & 62.6 & \textbf{66.2} \\
		\hline
        \multirow{3}{*}{WPR}                        & M-BERT            &- & - & 76.6 & - & 78.1 & 75.3 & 74.2 & - & 70.1 & 76.6 & - & - & - & - & - & - & 64.5 & 73.5 \\
		                                            & XLM-R$_{base}$           & - & - & 77.6 & - & 78.2 & 76.0 & 74.4 & - & 70.7 & 77.3 & - & - & - & - & - & - & 63.9 & 73.8 \\
		                                            & Unicoder   & - & - & 77.2 & - & 78.4 & 75.7 & 74.9 & - & 70.3 & 77.4 & - & - & - & - & - & - & 64.4 & 73.9 \\
		                                            &
		              CCPC   & - & - & 77.2 & - & 78.5 & 75.9 & 74.7 & - & 70.5 &  77.2 & - & - & - & - & - & - & 64.2 & \textbf{74.0} \\                          \hline    
        \multirow{3}{*}{QADSM}                        & M-BERT            &- & - & 60.3 & - & 68.3 & - & 64.1 & - & - &  - & - & - & - & - & - & - & - & 64.2 \\
		                                            & XLM-R$_{base}$           & - & - & 65.8 & - & 71.7 & - & 68.3 & - & - & - & - & - & - & - & - & - & - & 68.6 \\
		                                            & Unicoder   & - & - & 64.6 & - & 71.8 & - & 68.7 & - & - & - & - & - & - & - & - & - & - & 68.4 \\
		                                            &
		              CCPC   & - & - & 67.0 & - & 71.1 & - & 69.3 & - & - & - & - & - & - & - & - & - & - & \textbf{69.1} \\                          \hline    
        \multirow{3}{*}{XNLI}                        & M-BERT                 & 64.9                                & 68.9 & 71.1 & 66.4 & 82.1 & 74.3 &                                   73.8 & 60.0 & - &  - & 69.0 &                                   50.4 & 55.8 & 61.6 & 58.0 & 69.5 & 69.3                                & 66.3 \\
		                                            &
		                                                           Unicoder  & 68.5 & 73.2 & 71.6 & 71.6 & 82.9 & 75.0 & 74.7 & 66.0 & - & - & 70.6 & 64.1 & 67.0 & 68.7 & 62.5 & 71.2 & 69.7 & 70.5 \\
		                                            &
                                XLM-R$_{base}$            & 72.1 & 77.5 & 77.0 & 75.9 & 84.6 & 79.2 & 78.2 & 69.8 & - &  - & 75.5 & 64.7 & 71.6 & 72.9 & 65.1 & 74.8 & 73.7 & 74.2\\
		                                           & 
		                          		              CCPC   & 72.2 & 77.9 & 76.8 & 76.2 & 84.2 & 78.3 & 78.2 & 70.6 & - & - & 75.8 & 67.2 & 73.0 & 73.4 & 67.4 & 75.5 & 75.0 & \textbf{74.8} \\                          \hline    

	\end{tabular}
	}
	\caption{The overall evaluation results on cross-lingual understanding.
	}
	\label{tab:main-results} 
\end{table*}

\begin{table*}[!h]
  \small
	\centering
	\begin{tabular}{cccccccccccccccc}
		\hline
        \textbf{Model} & AR&AF&AM&AN&AZ&AS&AW&AE&BE&BD&BS&BR&BG&BN&CA  \\
%		\hline
		CCPC & 87.9&95.2&83.3&46.6&79.1&88.2&50.6&92.7&94.2&5.8&94.9&48.9&90.3&86.4&95.7      \\
        \hline
        
        \textbf{Model} & CB&CE&CS&CH&ZH&CR&CC&CY&DA&DE&DS&DT&EL&EO&ES  \\
%		\hline
		CCPC & 74.7&30.6&96.7&30.3&95.0&9.8&57.7&84.0&95.8&99.0&60.3&7.5&93.0&95.3&97.2      \\
       \hline
        
        
        \textbf{Model} & ET&EU&PS&FO&FI&FR&FY&GD&GA&GL&GS&HE&HI&HR&HS  \\
%		\hline
		CCPC & 94.8&89.5&93.8&79.8&96.5&94.9&90.5&72.9&82.4&94.8&62.8&90.8&96.2&96.7&68.8      \\
        \hline
        
        \textbf{Model} & HU&HY&IO&IE&IA&IL&ID&IT&JA&JV&KT&KB&KK&KO&KM  \\
%		\hline
		CCPC & 95.3&93.3&80.3&82.5&94.9&95.3&94.4&93.8&94.5&77.3&91.3&2.5&84.6&89.1&78.3      \\
        \hline
        
        \textbf{Model} & KU&KJ&LT&LN&LT&LS&ML&MR&MX&MH&MD&MN&NS&NO&NB  \\
%		\hline
		CCPC & 78.9&7.9&95.3&64.5&95.3&94.8&97.5&90.8&66.4&10.9&92.7&94.2&88.9&95.7&97.8      \\
        \hline
        
        \textbf{Model} & NV&OI&OR&PM&PR&PL&RO&SK&SV&SI&SP&SE&SG&NL&PT  \\
%		\hline
		CCPC & 71.2&72.5&50.8&11.0&58.4&97.0&96.7&95.7&93.9&94.8&93.8&95.8&81.7&97.0&95.0      \\
        \hline
        
        \textbf{Model} & RU&SW&TA&TE&TT&TK&TH&TL&TZ&UG&UK&UB&WR&WU&XO  \\
%		\hline
		CCPC & 93.5&64.2&89.1&94.4&75.8&30.8&95.3&89.0&49.5&86.5&93.8&68.7&30.1&83.2&45.1      \\
        \hline
        
        \textbf{Model} & YD&YU&ZM&TR&UR&VI&AVG&AVG$_{R}$&AVG$_{L}$&-&-&-&-&-&  \\
%		\hline
		CCPC & 88.4&88.7&95.8&97.1&91.3&96.3&78.8&65.5&83.7&-&-&-&-&-&      \\
        \hline
        
        
        
	\end{tabular}
	\caption{Evaluation results on English-aligned cross-lingual sentence retrieval. We present accuracy on all languages that Tatoeba supports. AVG$_{R}$ is the average accuracy of LASER, and AVG$_L$ is the average accuracy of LaBSE. The two scores are reported by \cite{feng2020language}}
	\label{tab:tatoeb_all} 
\end{table*}


\begin{table*}[!h]
  \small
	\centering
	\begin{tabular}{ccccccccccc}
		\hline
        \textbf{Model} & DE-PL&NL-FR&ZH-DE&DE-ZH&IT-RU&RU-JA&ZH-FR&FR-ZH&DE-IT&JA-FI  \\
%		\hline
		CCPC & 92.8&76.3&69.7&77.8&77.8&74.1&91.7&92.3&80.0&50.3      \\
        \hline
        
        \textbf{Model} & RU-IT&IT-DE&DE-UR&NL-DE&ES-UR&PT-FR&FR-NL&JA-RU&TR-ES&FR-PT  \\
%		\hline
		CCPC & 87.2&86.7&77.4&78.4&77.7&79.3&81.6&86.0&75.7&81.5      \\
       \hline
        
        
        \textbf{Model} & NL-ES&PL-JA&FR-UR&ES-TR&JA-PL&ES-JA&DE-NL&JA-ES&ES-NL&DE-HU  \\
%		\hline
		CCPC & 73.8&87.2&72.5&84.3&85.2&88.2&79.8&84.0&81.3&79.2      \\
        \hline
        
        \textbf{Model} & DE-JA&FR-JA&RU-ES&JA-FR&IT-FR&JA-DE&FR-ES&ES-FR&RU-DE&PT-ES  \\
%		\hline
		CCPC & 85.7&81.0&79.5&87.6&85.3&88.0&86.7&85.0&76.1&86.9      \\
        \hline
        
        \textbf{Model} & ES-PT&FR-IT&DE-RU&ES-RU&RU-FR&ES-DE&DE-ES&DE-FR&FR-DE&FR-RU  \\
%		\hline
		CCPC & 83.7&77.0&77.8&84.7&72.0&84.1&80.7&84.5&89.7&73.2      \\
        \hline
        
        
        
	\end{tabular}
	\caption{Evaluation results on non-English cross-lingual sentence retrieval. We select 50 language pairs that have most data in Tatoeba. }
	\label{tab:tatoeb_all} 
\end{table*}




We list some experiments on other cross-lingual downstreaming tasks, to illustrate that our model is able to handle some complex tasks such as MLQA, Web Page Ranking, XNLI etc. Given a task, each pretrained model is fine-tuned using its English training set only, and then applied to all test sets in different languages.

\paragraph{Cross-Lingual Understanding}
In the fine-tuning stage, the batch size is set to 32. We use Adam Optimizer~\cite{kingma2014adam} with warm-up and set the learning rate to 7e-6 and warm-up steps 10000. For all sentence classification tasks, we fine-tune 10 epochs.  For MLQA, we set the learning rate to 3e-5, batch size to 12 and train 2 epochs following BERT for SQuAD.
\begin{itemize}

\item MLQA:
The MLQA \cite{lewis2019mlqa} is a multilingual machine reading comprehension task, which contains QA annotations labeled in 7 languages, including \emph{English},  \emph{Arabic}, \emph{German}, \emph{Spanish}, \emph{Hindi}, \emph{Vietnamese} and \emph{Chinese}. 
F1 score of the predicted answers is used as the metric.


\item Web Page Ranking~(WPR)~\cite{liang-etal-2020-xglue}:
This task aims to predict whether a web page is relevant to an input query. 
It covers 7 languages, including \emph{English}, \emph{German}, \emph{French}, \emph{Spanish}, \emph{Italian}, \emph{Portuguese} and \emph{Chinese}. 
Each labeled instance is a 4-tuple: $<$query, web page title, web page snippet, label$>$. 
The relevance label contains 5 ratings: Perfect (4), Excellent (3), Good (2), Fair (1) and Bad (0). 
Normalize Discounted Cumulative Gain (nDCG) is used as the metric.


\item Query-Ad Matching (QADSM)\cite{liang-etal-2020-xglue}:
This task aims to predict whether an advertisement (ad) is relevant to an input query. 
It covers 3 languages, including \emph{English}, \emph{French} and \emph{German}. 
Each labeled instance is a 4-tuple: $<$query, ad title, ad description, label$>$.
The label indicates whether the ad is relevant to the query (Good), or not (Bad). 
Accuracy (ACC) of the binary classification is used as the metric.



\item XNLI:
We reuse the original XNLI dataset \cite{conneau2018xnli} in XGLUE.XNLI consists of 7500 human-annotated development and test examples in NLI three-way classification format in English,
French, Spanish, German, Greek, Bulgarian, Russian, Turkish, Arabic, Vietnamese, Thai, Chinese, Hindi, Swahili and Urdu, making a total of 112,500 annotated pairs. These languages span
several language families, and with the inclusion of Swahili and Urdu, include two lower-resource languages as well.




\end{itemize}

In Table\ref{tab:main-results}, we find CCPC has better performance on four tasks compared with Unicoder and XLM-R$_{base}$. Besides, we found CCPC has lower scores on English test set, while it's better than other models on other language which doesn't have any training corpus. When we focus on some low-resource language, such as sw, ur and hi, we can find CCPC can beat XLM-R$_{base}$ and Unicoder more significantly. These experiment results mean our model has strong and robust cross-lingual transfer ability.

\paragraph{Cross-Lingual Sentence Retrieval}
To exhibit the generalization of our model，we report all evaluation results on English-aligned cross-lingual sentence retrieval in table~\ref{tab:tatoeb_all}, which contains 110+ languages. We can found our model still has excellent performance on all languages. In table~\ref{tab:tatoeb_all}, we denote the average on all languages of LASER as AVG$_R$, and the average of all languages of LaBSE as AVG$_L$. It can be seen in table~\ref{tab:tatoeb_all} that our average accuracy~(78.8) is much higher than LASER(65.5), and it's close to LaBSE~(83.7). The excellent results of LaBSE come from two aspect. The first one is hardware. With TPU, LaBSE can be trained by 8192 batch size. The Second one is massive bilingual data. They collect bilingual corpus contains 6B translation pairs covering 109 languages. Compared with them, our results is more inspiring, because we trained our base model only with 64 batch size and large model with 32 batch size, and we don't rely on any bilingual corpus. 



